Chain-of-Knowledge: Integrating Knowledge Reasoning into Large Language Models by Learning from Knowledge Graphs

Large Language Models (LLMs) have exhibited impressive proficiency in various natural language processing (NLP) tasks, which involve increasingly complex reasoning. Knowledge reasoning, a primary type of reasoning, aims at deriving new knowledge from existing one.While it has been widely studied in the context of knowledge graphs (KGs), knowledge reasoning in LLMs remains underexplored. In this paper, we introduce Chain-of-Knowledge, a comprehensive framework for knowledge reasoning, including methodologies for both dataset construction and model learning. For dataset construction, we create KnowReason via rule mining on KGs. For model learning, we observe rule overfitting induced by naive training. Hence, we enhance CoK with a trial-and-error mechanism that simulates the human process of internal knowledge exploration. We conduct extensive experiments with KnowReason. Our results show the effectiveness of CoK in refining LLMs in not only knowledge reasoning, but also general reasoning benchmarkms.

==> Sections/5_Discussions.tex <==
\section{Discussions}

==> Tables/main_result.tex <==
\setlength\tabcolsep{7.5pt}
\begin{table*}[ht]
\small
  \centering
    \begin{tabular}{lllggggvvvv}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Rule Length}} & \multicolumn{4}{c}{\textbf{ID}} &  \multicolumn{4}{c}{\textbf{OOD}} \\
    \cmidrule(lr){4-7} \cmidrule(lr){8-11} 
    & & & \multicolumn{1}{c}{\textbf{2hop}} & \multicolumn{1}{c}{\textbf{3hop}} & \multicolumn{1}{c}{\textbf{4hop}} & \multicolumn{1}{c}{\textbf{all} }& \multicolumn{1}{c}{\textbf{2hop}} & \multicolumn{1}{c}{\textbf{3hop}} & \multicolumn{1}{c}{\textbf{4hop}} & \multicolumn{1}{c}{\textbf{all}} \\ 
    
    \midrule
    
    \multirow{10}{*}{Mistral-7b} 

        & Vanilla CoT & 
        - & 5.47 & 6.97 & 4.48 & 5.64 &
        4.98 & 5.47 & 4.98 & 5.14 \\

        \cmidrule(lr){2-11}
    
        & \multirow{3}{*}{Few-shot CoT} & 2hop &
        7.46 & 7.96 & 7.46 & 7.63 &
        7.96 & 6.97 & 6.97 & 7.30 \\
        
        & & 2+3 & 
        8.00 & 8.00 & 7.00 & 7.66 &
        8.50 & 7.00 & 7.00 & 7.33 \\
        
        & & 2+3+4 &
        6.50 & 7.00 & 7.50 & 7.00 & 
        7.00 & 5.00 & 7.50 & 6.50 \\

        \cmidrule(lr){2-11}
        
        & \multirow{3}{*}{CoK} & 2 &
        12.00 & 15.00 & 13.00 & 13.33 &
        17.00 & 8.00 & 6.00 & 10.33 \\

        & & 2+3 &
        16.00 & 20.00 & 17.00 & 17.66 &
        16.50 & 9.00 & 15.00 & 13.50 \\

        & & 2+3+4 & 
        13.50 & 16.00 & 22.00 & 17.16 &
        12.50 & 17.00 & 23.00 & 17.50 \\

        \cmidrule(lr){2-11}

        & \multirow{3}{*}{CoK(T\&E)} & 2 &
        12.00 & 9.00 & 10.00 & 10.33 &
        15.00 & 12.00 & 12.00 & 13.00 \\

        & & 2+3 & 
        18.50 & 25.00 & 17.00 & 20.16 &
        21.00 & 24.00 & 20.00 & 21.66 \\

        & & 2+3+4 &
        15.00 & 18.00 & 23.00 & 18.66 &
        18.50 & 20.00 & 26.00 & 21.50 \\

    \midrule 
    
    \multirow{10}{*}{Llama3-8B}

        & Vanilla CoT & - &
        5.00 & 7.00 & 9.00 & 7.00 &
        6.00 & 9.00 & 6.00 & 7.00 \\

        \cmidrule(lr){2-11}

        & \multirow{3}{*}{Few-shot CoT}
        & 2 &
        - & - & - & - &
        - & - & - & -\\

        & & 2+3 &
        - & - & - & - &
        - & - & - & -\\

        & & 2+3+4 &
        - & - & - & - &
        - & - & - & -\\

        \cmidrule(lr){2-11}

        & \multirow{3}{*}{CoK}
        & 2 &
        17.50 & 13.00 & 14.00 & 14.83 &
        13.50 & 9.00 & 8.00 & 10.16 \\

        & & 2+3 &
        15.50 & 20.00 & 14.00 & 16.50 &
        19.50 & 16.00 & 15.00 & 16.83 \\

        & & 2+3+4 &
        16.50 & 19.00 & 22.00 & 19.16 &
        10.50 & 18.00 & 20.00 & 16.16 \\

        \cmidrule(lr){2-11}

        & \multirow{3}{*}{CoK(T\&E)}
        & 2 &
        12.00 & 16.00 & 16.00 & 14.66 &
        19.00 & 17.00 & 12.00 & 16.00 \\

        & & 2+3 &
        12.00 & 21.00 & 17.00 & 16.66 & 
        21.50 & 24.00 & 19.00 & 21.50 \\

        & & 2+3+4 &
        17.00 & 20.00 & 21.00 & 19.33 &
        13.00 & 22.00 & 23.00 & 19.33 \\
    
    
    \bottomrule
    \end{tabular}
  \caption{results of the anonymized experiment}
  \label{tab:main_result}
\end{table*}
